Bias Beyond English: Counterfactual Tests for Bias in Sentiment Analysis in Four Languages

Sentiment analysis (SA) systems are used in many products and hundreds of languages. Gender and racial biases are well-studied in English SA systems, but understudied in other languages, with few resources for such studies. To remedy this, we build a counterfactual evaluation corpus for gender and racial/migrant bias in four languages. We demonstrate its usefulness by answering a simple but important question that an engineer might need to answer when deploying a system: What biases do systems import from pre-trained models when compared to a baseline with no pre-training? Our evaluation corpus, by virtue of being counterfactual, not only reveals which models have less bias, but also pinpoints changes in model bias behaviour, which enables more targeted mitigation strategies. We release our code and evaluation corpora to facilitate future research.

==> figures/all_results.tex <==
% TODO work out how to put the language labels and the bias types on them without lots of captions? OR maybe captions are good.
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_ja_gender.pdf}
        \caption{Japanese (ja) - Gender}
        \label{fig:ja_gender}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_ja_race.pdf}
        \caption{Japanese (ja) - Race}
        \label{fig:ja_race}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_zh_gender.pdf}
        \caption{Chinese (zh) - Gender}
        \label{fig:zh_gender}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_de_gender.pdf}
        \caption{German (de) - Gender}
        \label{fig:de_gender}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_de_race.pdf}
        \caption{German (de) - Race}
        \label{fig:de_race}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_es_gender.pdf}
        \caption{Spanish (es) - Gender}
        \label{fig:es_gender}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_es_race.pdf}
        \caption{Spanish (es) - Race}
        \label{fig:es_race}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_en_gender.pdf}
        \caption{English (en) - Gender}
        \label{fig:en_gender}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_en_race.pdf}
        \caption{English (en) - Race}
        \label{fig:en_race}
    \end{subfigure}
    % TODO can I put en_scrubbed on the same graph as en? Have either 8 or 10 graphs depending which...

    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Mean and variance of difference in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}). Monolingual models are trained and tested on the same language, multilingual models are pretrained multilingual models where the classification layer is trained on English and then zero shot to the target language.} 
    \label{fig:all_results}
\end{figure*}


% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[b]{0.348\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_baseline.pdf}
%         \caption{Baseline (monolingual) models}
%         \label{fig:baseline_results}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_mono.pdf}
%         \caption{Monolingual models}
%         \label{fig:mono_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%       %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_multi.pdf}
%         \caption{Multilingual models}
%         \label{fig:multi_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%     %(or a blank line to force the subfigure onto a new line)
   
%     \caption{Mean performance gap between privileged and minoritized groups, by language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias. Languages are ISO codes, with \textit{en\_s} for English (scrubbed). Points that are not statistically significant ($\alpha < 0.05$) are included but marked with an X. Monolingual models are trained and tested on the same language, multilingual model are pretrained mbert models where the classification layer is trained on English and then zero shot to the target language.} 
%     \label{fig:all_results}
% \end{figure*}


==> figures/all_results_violin.tex <==
% TODO work out how to put the language labels and the bias types on them without lots of captions? OR maybe captions are good.
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_ja_gender.pdf}
        \caption{Japanese (ja) - Gender}
        \label{fig:ja_gender_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_ja_race.pdf}
        \caption{Japanese (ja) - Race}
        \label{fig:ja_race_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_zh_gender.pdf}
        \caption{Chinese (zh) - Gender}
        \label{fig:zh_gender_violin}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_de_gender.pdf}
        \caption{German (de) - Gender}
        \label{fig:de_gender_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_de_race.pdf}
        \caption{German (de) - Race}
        \label{fig:de_race_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_es_gender.pdf}
        \caption{Spanish (es) - Gender}
        \label{fig:es_gender_violin}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_en_gender.pdf}
        \caption{English (en) - Gender}
        \label{fig:en_gender_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_en_race.pdf}
        \caption{English (en) - Race}
        \label{fig:en_race_violin}
    \end{subfigure}
    % TODO can I put en_scrubbed on the same graph as en? Have either 8 or 10 graphs depending which...

    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Violin plots of the distribution of differences in sentiment label under each counterfactual (range is -4 to 4 since labels range from 1 to 5). Higher numbers indicate greater bias against the minoritized group, 0 indicates invariance to the counterfactual. Monolingual models are trained and tested on the same language, multilingual models are pretrained multilingual models where the classification layer is trained on English and then zero shot to the target language.} 
    \label{fig:all_results_violin}
\end{figure*}


% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[b]{0.348\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_baseline.pdf}
%         \caption{Baseline (monolingual) models}
%         \label{fig:baseline_results}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_mono.pdf}
%         \caption{Monolingual models}
%         \label{fig:mono_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%       %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_multi.pdf}
%         \caption{Multilingual models}
%         \label{fig:multi_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%     %(or a blank line to force the subfigure onto a new line)
   
%     \caption{Mean performance gap between privileged and minoritized groups, by language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias. Languages are ISO codes, with \textit{en\_s} for English (scrubbed). Points that are not statistically significant ($\alpha < 0.05$) are included but marked with an X. Monolingual models are trained and tested on the same language, multilingual model are pretrained mbert models where the classification layer is trained on English and then zero shot to the target language.} 
%     \label{fig:all_results}
% \end{figure*}


==> figures/baseline_mono_confusion_matrix.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/confusion_matrix/baseline_mono_heatmap.pdf}
    \caption{Confusion matrices for racial demographic counterfactual pairs for Japanese and German, comparing the difference between baseline and monolingual transfer (mono-T) models (RQ1). Higher colour saturation in the lower triangle is bias against the minoritised group, in the upper triangle is bias against the privileged group. Other languages and bias types follow the same pattern between baseline and mono-T models (regardless of absolute level of bias).} 
    \label{fig:baseline_mono_conf_matrix}
    \vspace{-1em}
\end{figure}

==> figures/baseline_mono_confusion_matrix_old.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_race_baseline_cap.pdf}
        \caption{Japanese (ja) Baseline}
        \label{fig:ja_race_baseline_conf}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_race_mono_cap.pdf}
        \caption{Japanese (ja) Mono-T}
        \label{fig:ja_race_mono_conf}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
   
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/de_race_baseline_cap.pdf}
        \caption{German (de) Baseline}
        \label{fig:de_race_baseline_conf}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/de_race_mono_cap.pdf}
        \caption{German (de) Mono-T}
        \label{fig:de_race_mono_conf}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \caption{Confusion matrices for racial demographic counterfactual pairs for Japanese and German, comparing the difference between baseline and monolingual transfer (Mono-T) models. Higher colour saturation in the lower triangle is bias against the minoritised group, in the upper triangle is bias against the privileged group. Data along the matrix diagonal (invariance under the counterfactual) has been removed to make interpretation clearer, as even in the most biased models many samples are invariant. Other languages and bias types follow the same pattern between baseline and Mono-T models (regardless of absolute level of bias).} 
    \label{fig:baseline_mono_conf_matrix}
    \vspace{-1em}
\end{figure*}


%ig:baseline_mono_conf_matrix

==> figures/baseline_vs_mono_old.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/baseline_vs_mono_agg.pdf}
    \caption{Aggregate bias metrics for baseline (blue), mono-T (orange), and distil mono-T (green) models: mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:baseline_vs_mono_old}
    \vspace{-1em}
\end{figure*}


==> figures/compressed_agg.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/aggregate/compression_gender.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/aggregate/compression_race.pdf}
    \end{subfigure}
   
    \caption{Aggregate bias metrics (RQ2): Comparison of mono-T (blue), and distil-mono-T (orange), ZS-XLT (green), and distil-ZS-XLT (red). Mean
and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type
of bias tested. mono-T and ZS-XLT models are repeated from Fig~\ref{fig:mono_vs_multi} to enable easier visual comparison to distilled models. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates
no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:compressed_agg}
    \vspace{-1em}
\end{figure*}

==> figures/en_scrubbed_results.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.46\textwidth}
        \includegraphics[width=\textwidth]{figures/compare_langs/compare_langs_en_en_scrubbed_gender_errbars.pdf}
        \caption{Mean and variance of the performance gaps for the gender counterfactuals in monolingual models of English (O) and scrubbed English (X). Positive numbers are bias against the minoritised group (in this case, female), 0 is no bias, and negative is bias against the privileged group. Shaded region represents 3\% of total range (see \ref{sec:metrics}).}
        \label{fig:en_scrubbed_errbars}
    \end{subfigure}
    \begin{subfigure}[b]{0.46\textwidth}
        \includegraphics[width=\textwidth]{figures/compare_langs/compare_langs_en_en_scrubbed_baseline_gender.pdf}
        \caption{Difference between confusion matrices of the gender counterfactual for English and scrubbed English baseline model (male demographic labels on x axis, female demographic counterfactual on y). The diagonal represents no bias in either direction, the upper right is bias against men, the lower left is bias against women. Red cells mean the English model has more, blue mean the scrubbed English model has more, and white mean their numbers are identical.}
        \label{fig:diff_matrix_en_scrubbed}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Comparisons of gender bias for English and English with explicit gender identifiers removed (aka "scrubbed" English). Scrubbing increases bias in the baseline, but does not much change either neural model.} 
    \label{fig:en_scrubbed_experiments}
\end{figure}


==> figures/fig_template.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.348\textwidth}
        \includegraphics[width=\textwidth]{figures/X.pdf}
        \caption{}
        \label{fig:b}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/Y.pdf}
        \caption{}
        \label{fig:}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/X.pdf}
        \caption{}
        \label{fig:}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{} 
    \label{fig:}
\end{figure*}


==> figures/front_example.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/front_example_long.pdf}
    \caption{We use counterfactual evaluation to evaluate how bias is differs in monolingual vs. cross-lingual systems. Counterfactual pairs (e.g. sentences \textit{a}, \textit{b}) vary a single demographic variable (e.g. race). We measure bias as the difference in scores for the pair. An unbiased model should be invariant to the counterfactual, with a difference of zero.}
    \label{fig:front_example}
    \vspace{-1em}
\end{figure}

==> figures/label_bal_confusion.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.215\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_gender_multi_xl_c_cap.pdf}
        \caption{distil ZS-XLT* (not balanced)}
        \label{fig:distilZSXLT_confusion}
    \end{subfigure}
    \begin{subfigure}[b]{0.215\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_gender_multi_xl_c_b_cap.pdf}
        \caption{distil ZS-XLT (balanced)}
        \label{fig:distilZSXLT_balanced_confusion}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Confusion matrices for gender counterfactual pairs for Japanese, comparing the difference between a model trained with imbalanced and balanced labels. Higher colour saturation in the lower triangle is anti-female bias, in the upper is anti-male. Data along the matrix diagonal (no change under counterfactual) has been removed to make interpretation clearer. Other languages and bias types follow the same visual pattern of the matrix between balanced and imbalanced labels, regardless of of distillation and of absolute level of bias.} 
    \label{fig:label_balancing_confusion}
    \vspace{-1em}
\end{figure}


==> figures/mono_vs_multi.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/aggregate/mono_multi_gender.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/aggregate/mono_multi_race.pdf}
    \end{subfigure}
   
    \caption{Aggregate bias metrics (RQ1): Comparison of mono-T (blue), and mono-XLT (orange), ZS-XLT (green). Mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:mono_vs_multi}
    \vspace{-1em}
\end{figure*}




==> figures/mono_vs_multi_old.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/mono_vs_multi_agg.pdf}
    \caption{Aggregate bias metrics for mono-T (blue), and mono-XLT (orange), ZS-XLT (green), distil mono-T (red), and distil ZS-XLT (purple) models. Mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:mono_vs_multi_old}
    \vspace{-1em}
\end{figure*}


==> figures/new_confusion_gender.tex <==
\begin{figure}[ht]
    \centering
        \begin{subfigure}[b]{0.48\textwidth}
        \caption{Japanese (ja) Gender}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_gender_heatmap.pdf}
        \label{subfig:ja_gender_conf}
    \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.48\textwidth}
        \caption{Chinese (zh) Gender}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/zh_gender_heatmap.pdf}
        \label{subfig:zh_gender_conf}
    \end{subfigure}
           ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.48\textwidth}
        \caption{German (de) Race}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/de_race_heatmap.pdf}
        \label{subfig:de_race_conf}
    \end{subfigure}
    \caption{Example confusion matrices for demographic counterfactual pairs for gender in Japanese and Chinese and race in German. From left to right: mono-T models, mono-XLT models, and ZS-XLT models.  \textbf{++} to \textbf{-{}-} are sentiment scores. Rows are predicted sentiment scores for the privileged group, columns predicted scores for the minoritised group. Higher colour saturation in the lower triangle is bias against the minoritised group, in the upper triangle is bias against the privileged group. Colour saturations are different scales for different models. Not visualised here: actual (ground-truth) sentiment scores.} 
    \label{fig:ja_zh_de_conf_matrix}
    \vspace{-1em}
\end{figure}

==> figures/normal_vs_balanced.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/label_bal_agg.pdf}
    \caption{Aggregate bias metrics for label balancing experiments:. Mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:normal_vs_balanced}
    \vspace{-1em}
\end{figure*}


==> tables/in_domain_performance_long.tex <==
% !TEX root = ../acl.tex


\begin{table}[h]
\adjustbox{max width=0.5\textwidth}{%
\centering
\begin{tabular}{llllll}
& \multicolumn{2}{c}{\textbf{Standard}}  & \multicolumn{2}{c}{\textbf{Distilled}}  \\
& F1 & Steps & F1 & Steps  \\
\toprule
ja & \textbf{0.62} & 44370 & 0.61 & 60436  \\
zh & \textbf{0.56} & 35190 & 0.53 & 43750  \\
de & \textbf{0.63} & 36720 & 0.63 & 52621  \\
es & \textbf{0.61} & 41310 &  & -  \\
en & \textbf{0.65} & 27050 & \textbf{0.65} & 44285  \\
%en\_s & \textbf{0.65} & 26520 & 0.64 & 17193 & 0.52 \\
%multi & \textbf{0.71} & 100644 & 0.70 & 78280 & - \\
ZS-XLT & \textbf{0.69} & 75000 & 0.68 & 33336  \\

\bottomrule
\end{tabular}
}
    \caption{F1 at convergence and steps at convergence for standard size and distilled models. Monolingual model performance is measured on the MARC data, ZS-XLT model performance on the US reviews data.}
    \label{tab:in_domain_performance_long}
\end{table}


==> tables/tab_template.tex <==
% !TEX root = ../acl.tex


\begin{table}[h]
\adjustbox{max width=\textwidth}{%
\centering
\begin{tabular}{lllllll}
& X & Y \\
\toprule
ja &  &  &  & &  & \\
zh &  &  &  & &  & \\
de &  &  &  & &  & \\
es &  &  &  & &  & \\
en &  &  &  & &  & \\
en_s &  &  &  & &  & \\
multi &  &  &  & &  & \\
multi-bal &  &  &  & &  & \\

\bottomrule
\end{tabular}
}
    \caption{Blah}
    \label{tab:}
\end{table}
